CHAMELEON: A Deep Learning Meta-Architecture for News Recommender Systems [Phd. Thesis]

Recommender Systems (RS) have became a popular research topic and, since 2016, Deep Learning methods and techniques have been increasingly explored in this area. News RS are aimed to personalize users experiences and help them discover relevant articles from a large and dynamic search space. The main contribution of this research was named CHAMELEON, a Deep Learning meta-architecture designed to tackle the specific challenges of news recommendation. It consists of a modular reference architecture which can be instantiated using different neural building blocks. As information about users' past interactions is scarce in the news domain, the user context can be leveraged to deal with the user cold-start problem. Articles' content is also important to tackle the item cold-start problem. Additionally, the temporal decay of items (articles) relevance is very accelerated in the news domain. Furthermore, external breaking events may temporally attract global readership attention, a phenomenon generally known as concept drift in machine learning. All those characteristics are explicitly modeled on this research by a contextual hybrid session-based recommendation approach using Recurrent Neural Networks. The task addressed by this research is session-based news recommendation, i.e., next-click prediction using only information available in the current user session. A method is proposed for a realistic temporal offline evaluation of such task, replaying the stream of user clicks and fresh articles being continuously published in a news portal. Experiments performed with two large datasets have shown the effectiveness of the CHAMELEON for news recommendation on many quality factors such as accuracy, item coverage, novelty, and reduced item cold-start problem, when compared to other traditional and state-of-the-art session-based recommendation algorithms.

==> Cap3/cap3-additionalrefs.tex <==

\section{Additional readings}

\subsection{What to Do Next: Modeling User Behaviors by Time-LSTM}
TODO: Desenvolver de \cite{zhunext2017}

Recently, Recurrent Neural Network (RNN) solutions
for recommender systems (RS) are becoming
increasingly popular. The insight is that, there exist
some intrinsic patterns in the sequence of users’
actions, and RNN has been proved to perform excellently
when modeling sequential data. In traditional
tasks such as language modeling, RNN solutions
usually only consider the sequential order
of objects without the notion of interval. However,
in RS, time intervals between users’ actions are of
significant importance in capturing the relations of
users’ actions and the traditional RNN architectures
are not good at modeling them. In this paper, we
propose a new LSTM variant, i.e. Time-LSTM,
to model users’ sequential actions. Time-LSTM
equips LSTM with time gates to model time intervals.
These time gates are specifically designed,
so that compared to the traditional RNN solutions,
Time-LSTM better captures both of users’ shortterm
and long-term interests, so as to improve the
recommendation performance. Experimental results
on two real-world datasets show the superiority
of the recommendation method using TimeLSTM
over the traditional methods.

%Code using Theano: https://github.com/DarryO/time_lstm

\subsection{Recurrent coevolutionary latent feature processes for continuous-time recommendation}
Desenvolver de \cite{dai2016recurrent}

Matching users to the right items at the right time is a fundamental task in recommender systems. As users interact with different items over time, users' and items' feature may drift, evolve and co-evolve over time. Traditional models based on static latent features or discretizing time into epochs can become ineffective for capturing the fine-grained temporal dynamics in the user-item interactions. We propose a coevolutionary latent feature process model that accurately captures the coevolving nature of users' and items' feature. We use a recurrent neural network to automatically learn a representation of influences from drift, evolution and co-evolution of user and item features. We develop an efficient stochastic gradient algorithm for learning the model parameters which can readily scale up to millions of events. Experiments on diverse real-world datasets demonstrate significant improvements in user behavior prediction compared to state-of-the-arts.


\subsection{Deep Coevolutionary Network: Embedding User and Item Features for Recommendation}
TODO: Desenvolver de \cite{dai2017deep}

Recommender systems o=en use latent features to explain the behaviors
of users and capture the properties of items. As users
interact with dierent items over time, user and item features can
in=uence each other, evolve and co-evolve over time. e compatibility
of user and item’s feature further in=uence the future
interaction between users and items.
Recently, point process based models have been proposed in
the literature aiming to capture the temporally evolving nature of
these latent features. However, these models o=en make strong
parametric assumptions about the evolution process of the user
and item latent features, which may not re=ect the reality, and has
limited power in expressing the complex and nonlinear dynamics
underlying these processes.
To address these limitations, we propose a novel deep coevolutionary
network model (DeepCoevolve), for learning user and
item features based on their interaction graph. DeepCoevolve use
recurrent neural network (RNN) over evolving networks to de=ne
the intensity function in point processes, which allows the model
to capture complex mutual in=uence between users and items, and
the feature evolution over time. We also develop an ecient procedure
for training the model parameters, and show that the learned
models lead to signi=cant improvements in recommendation and activity
prediction compared to previous state-of-the-arts parametric
models.

\subsection{Temporal learning and sequence modeling for a job recommender system}
TODO: Desenvolver de \cite{liu2016temporal}

We present our solution to the job recommendation task for RecSys Challenge 2016. The main contribution of our work is to combine temporal learning with sequence modeling to capture complex user-item activity patterns to improve job recommendations. First, we propose a time-based ranking model applied to historical observations and a hybrid matrix factorization over time re-weighted interactions. Second, we exploit sequence properties in user-items activities and develop a RNN-based recommendation model. Our solution achieved 5th place in the challenge among more than 100 participants. Notably, the strong performance of our RNN approach shows a promising new direction in employing sequence modeling for recommendation systems.



\subsection{Click-Through Rate prediction}

\subsubsection{Wide \& Deep Learning for Recommender Systems}
TODO: Desenvolver de \cite{cheng2016wide}

\subsubsection{DeepFM: A Factorization-Machine based Neural Network for CTR Prediction}
TODO: Desenvolver de \cite{guo2017deepfm}
%Tensorflow code: https://github.com/Leavingseason/OpenLearning4DeepRecsys




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


Refugo do Cap 3


\subsection{From Word Embeddings to Item Recommendation}

TODO: Summarize from \cite{ozsoy2016} (ver resumo docs)

\subsection{Word embedding based retrieval model for similar cases recommendation}

TODO: Summarize from \cite{zhao2015word}






\subsection{Restricted Boltzman Machines for Collaborative Filtering}

Early pioneer work which used neural network was done in \cite{salakhutdinov2007}. They introduced a two-layer Restricted Boltzmann Machines (RBM) to model ratings. Since maximum likelihood estimation is intractable in these models, they show that optimization can be done efficiently by following an approximation to the gradient of a different objective function \cite{zheng2016}. 

A RBM model is trained for each user, and the visible softmax units corresponds with the items rated by the user, as shown in Figure \ref{figure:rbmarch}. If user \textit{a} and user \textit{b} rated the same item, their RBMs share weights connected to the corresponding visible unit \cite{zheng2016}. This consists in an advantage for computational tractability.

\begin{figure}[h]
	\centering
	\includegraphics[height=7cm]{Cap3/rbm_rec_arch.png}
	\caption{Architecture of a RBM for a user \cite{zheng2016}}
	\label{figure:rbmarch}
\end{figure}

Although the authors in \cite{salakhutdinov2007} show that RBM can be successfully applied to the recommendation problem and slightly outperforms traditional Matrix Factorization, the proposed model is not deep enough and only consists of 2 layers. Learning deep models has been successfully applied in the domain of modeling temporal data \cite{bengio2003} \cite{pan2008} and learning word embedding \cite{mikolov2013} \cite{turian2010}. Training a deeper RBM is helpful for capturing hierarchical latent factors of users and items and more accurately modeling ratings \cite{zheng2016}.

RBM does not make use of content information, such as user profiles or review texts \cite{zheng2016}. As a result, the proposed model cannot deal with the cold start problem \cite{schein2002}, where recommender systems are required to give recommendations to novel users who have no preference on any items, or recommending items that no user of the community has rated yet  \cite{zheng2016}. 

RBM targets rating prediction, not top-N recommendation, and its loss function considers only the observed ratings. It is technically challenging to incorporate negative sampling, which would be required for top-N recommendation, into the training of RBM. For this reason, we do not compare with RBM in our experiments, but test several other neural network baselines that work for top-N recommendation \cite{wu2016}.







\subsection{Autoencoders for recommendation}

Recently autoencoders have become a popular choice for building recommendation systems \cite{chen2012}\cite{sedhain2015}\cite{strub2015}. The idea of user-based AutoRec \cite{sedhain2015} is to learn hidden structures that can reconstruct a user's ratings given her historical ratings as inputs. In terms of user personalization, this approach shares a similar spirit as the item-item model \cite{ning2011}\cite{sarwar2001} that represent a user as her rated item features. While previous work has lent support for addressing collaborative filtering, most of them have focused on observed ratings and modeled the observed data only. As a result, they can easily fail to learn users preference from the positive-only implicit data.

A subclass of deep CF methods use denoising autoencoders as the central component of their model, as can be seeing in this section.


To utilize information from text, \cite{wang2015} integrates an autoencoder and Probabilistic Matrix Factorization (PMF). Item text is represented by using bag-of-words and taken as input to the autoencoder to learn item features. User features are modeled by a Gaussian distribution. However, they do not jointly model users and items from text. In addition, this approach is only suitable for one-class collaborative filtering problems \cite{pan2008} \cite{zheng2016} 

\subsubsection{Collaborative Deep Learning (CDL)}.
In \cite{wang2015}, it was introduced a technique named Collaborative Deep Learning (CDL), which utilizes review texts along with ratings, in order to address the cold start problem. They integrate a bayesian Stack Denoise Auto Encoder (SDAE) \cite{vincent2010} and Collaborative Topic Regression (CTR) \cite{wang2011}. It learns latent factors of items from review texts and draw a latent user vector from Gaussian distribution \cite{zheng2016}. CDL uses tags and metadata instead of the item ID. CDL was the first deep model to learn from review texts for recommender systems \cite{betru2017}.

In \cite{zheng2016}, some critiques for the work of \cite{wang2015} are presented. First, Collaborative Deep Learning only models item review texts. In recommender systems, user provides reviews to express their feelings. These review texts can be utilized to learn preference of users. 

Second, review texts are represented by using bag of words scheme. As we know, bag of words vectors only convey the frequency of words. If two reviews are semantically related but use different words, CDL, which uses bag-of-words, may not consider the two reviews to be similar . The vocabulary in English is very diverse and two reviews can be semantically similar even with low lexical overlap, so semantic meaning is especially important \cite{zheng2016}. However, semantic meanings, which are essential for reveal user attitudes and item properties, are lost in CDL. 

At last, in Collaborative Deep Learning, word order is ignored. However, in many text modeling applications, word order is extremely important \cite{wallach2006}. To further improve the performance of Collaborative Deep Learning, word order should be taken into consideration while modeling review texts \cite{betru2017}.

\subsection{Deep collaborative filtering via marginalized denoising auto-encoder}

In \cite{li2015deep}, authors propose a general deep architecture named Deep Collaborative Filtering (DCF), shown in Figure \ref{figure:dcf}, which integrates matrix factorization and deep feature learning. It models the mappings between the latent factors used in CF and the latent layers in deep models.
They also present a practical instantiation of the proposed architecture, by utilizing the probabilistic matrix factorization and Marginalized Denoising Auto-encoders (mDA) \cite{chen2012}. The scalability and low computational cost of the mDA makes it an interesting approach.

Unlike \cite{wang2015} which integrates collaborative topic regression and bayesian stacked denoising auto-encoders and requires learning of a large number of hyper parameters using an EM style algorithm, their approach uses a ore efficient architecture based upon mDA and stochastic gradient descent and is more computationally efficient and scalable.


\begin{figure}[h]
	\centering
	\includegraphics[height=7cm]{Cap3/dcf_architecture.png}
	\caption{DCF general framework in \cite{li2015deep}}
	\label{figure:dcf}
\end{figure}


\subsubsection{Collaborative filtering with stacked denoising autoencoders and sparse inputs}
TODO:Summarize from \cite{strub2015}

\subsubsection{Collaborative topic modeling for recommending scientific articles}
TODO:Summarize from \cite{wang2011}

From \cite{wu2016}...
Another related work is [27], which also uses the Auto-Encoder
for recommender systems. This work studies the particular prob-
lem of article recommendation, and improves the well-known model
Collaborative Topic Regression [26] by replacing its Topic Model
component by a Bayesian Auto-Encoder, which is used for learn-
ing the latent feature representations for the articles. Different from
this model, our model is a generic model and addresses the general
top-N recommendation problem, and the inputs are user behaviors
instead of item/article features.

\subsubsection{Autorec: Autoencoders meet collaborative filtering}
TODO: Summarize from \cite{sedhain2015}

From \cite{wu2016}...
We are aware of a concurrent proposal called AutoRec [20],
which uses the Auto-Encoder for rating prediction. The main dif-
ferences are as follows: 1) AutoRec only considers the observed
ratings in the loss function, which does not guarantee the perfor-
mance for top-N recommendation. 2) They use the vanilla Auto-
Encoder structure, while we prove that introducing user factors in
the model can greatly improve performance. 3) AutoRec does not
employ the denoising technique, which is a major part of our work.


\subsubsection{Collaborative Denoising Auto-Encoders for top-n recommender systems (CDAE)}

Learning from intentionally corrupted input has been widely studied. In \cite{wu2016}, a method for top-N recommendation named Collaborative Denoising Auto-Encoder (CDAE) is presented. It is probably the first work to utilize, for recommender systems, the idea of Denoising Auto-Encoders (DAE) \cite{vincent2008extracting}. DAE extends the classical auto-encoder by training to reconstruct each data point x from its (partially) corrupted version. The goal of DAE is to force the hidden layer to discover more robust features and to prevent it from simply learning the identity function.

\begin{figure}[h]
	\centering
	\includegraphics[height=7cm]{Cap3/cdae.png}
	\caption{A sample CDAE illustration for a user \textit{u} \cite{wu2016}}
	\label{figure:cdae}
\end{figure}

CDAE, shown in Figure \ref{figure:cdae} assumes that whatever user-item interactions are a corrupted version of the user's full preference set. The model learns latent representations of corrupted user-item preferences that can best reconstruct the full input, recovering co-preference patterns. It uses an additional user node on the input and bias node beside the hidden layer.

\subsubsection{Collaborative Recurrent Autoencoder (CRAE)}
TODO: 

CRAE [Wang et. al, 2016]
Collaborative Recurrent Autoencoder
Encodes text (e.g. movie plot, review)
Autoencoding with RNNs
- Encoder-decoder architecture
- The input is corrupted by replacing words with a deisgnated
BLANK token
CDL model + text encoding simultaneously
- Joint learning

[Wang et. al, 2016] H. Wang, X. Shi, DY. Yeung: Collaborative Recurrent Autoencoder: Recommend while Learning to Fill in the Blanks. Advances in Neural Information
Processing Systems (NIPS 2016)


\subsection{Neural collaborative filtering}

TODO: Summarize from \cite{he2017}

%Code: https://github.com/hexiangnan/neural_collaborative_filtering


\subsubsection{Other Deep CF methods}

Coevolving features [Dai et. al, 2016]
- Users' taste and items' audiences change over time (e.g. forum discussions)
- User/item features depend on time
- User/item features are composed of
-- Time drift vector
-- Self evolution
-- Co-evolution with items/users
-- Interaction vector
- Feature vectors are learned by RNNs


Product Neural Network (PNN) [Qu et. al, 2016]
- For CTR estimation
- Embedded features
- Pairwise layer: all pairwise combination of embedded features
-- Like Factorization Machines
-- Outer/inner product of feature vectors or both
- Several fully connected layers


 CF-NADE [Zheng et. al, 2016] \cite{zheng2016autoregressive}
- Neural Autoregressive Collaborative Filtering
- User events reference (0/1) + confidence (based on occurence)
- Reconstructs some of the user events based on others (not the full set)
-- Random ordering of user events
-- Reconstruct the preference i, based on preferences and confidences up to i-1
- Loss is weighted by confidences
(ver resumo docs) See also http://tech.hulu.com/blog/2016/08/01/cfnade.html






==> Cap4/cap4-notes.tex <==

%	\item Recommendation objective: Maximize the users personalized ranking utility of top-n recommendations.

\subsection{Main inspirations}

\begin{itemize}
	\item Session-based: LSTM \cite{lee2016quote} LSTM/GRU bidirectional with attention \cite{kumar2017} with Variational Dropout \cite{gal2016theoretically} / zoneout \cite{krueger2016zoneout} or 3D CNN \cite{tuan20173d}. Dilated Recurrent Neural Networks: %https://arxiv.org/abs/1710.02224?utm_campaign=Revue%20newsletter&utm_medium=Newsletter&utm_source=NLP%20News
	\item Session splitting: When the actual session is not available, artificially split using heuristics like in \cite{gayo2009survey}
	\item Item IDS representation: OHE ids or embedding (map one-hot vectors into a
	densified information space) \cite{mikolov2013efficient} \cite{mikolov2013distributed} embedding dropout \cite{tan2016improved}. Pre-train user and item embeddings in a simple network (eg. DSSM) \cite{song2016multi}. Add item-specific embedding (based on a previous matrix factorization) to textual embedding when available and 0 when not available \cite{bansal2016ask}
	\item Text representation learning: doc2vec \cite{kumar2017}, RNN on Word2Vec/Glove \cite{bansal2016ask}, CNN on Word2Vec/Glove \cite{lee2016quote} \cite{catherine2017transnets}, CNN with Dual Local-Global Attention \cite{seo2017interpretable} or character-level CNN \cite{tuan20173d}	
	\item User IDs representation: embedding from OHE directly included in the RNN gated cell \cite{donkers2017sequential}
	\item Inter-session: using previous session hidden state to initialize GRU in the new session \cite{ruocco2017inter} or hierarquical RNNs to model user cross-sessions \cite{quadrana2017personalizing}. Use separate RNNs to model user behaviour across time at different rates (eg. daily, weekly) \cite{song2016multi}.
	\item Contextual features: Categorical features (category)  \cite{tuan20173d} time since last event, discretized timestamp (month, day, hour) using adaptive context-specific input/transition matrices\cite{liu2016context} or a Context Wrapper for GRU cell \cite{smirnova2017contextual}
	\item Item-side features: Publisher/source, tags/category, creationDate
	\item Multi-task learning: Predict item-side features (eg. publisher, categories, user location) \cite{bansal2016ask}, statistics (eg. Avg CTR). Use future information about the session (not available at runtime) to improve training. More on Multi-Task Learning in http://ruder.io/multi-task/index.html / http://ruder.io/multi-task-learning-nlp/index.html
	Privileged information: Leverage subsequent items users has visited in the session \cite{tan2016improved}
	\item Joining layer: Factorization Machine for interaction of user and item learned representation \cite{zheng2017joint} \cite{catherine2017transnets}, feedforward layer \cite{hidasi2016} \cite{hidasi2017}, deep crossing for similarity layer \cite{shan2016deep}, cosine similarity \cite{kumar2017}, \cite{elkahky2015multi}. Cosine similarity and WARP loss \cite{weston2014tagspace}
	\item Ouput: CTR (logistic log loss) with negative sampling  \cite{bansal2016ask}, softmax on cosine loss \cite{elkahky2015multi} \cite{kumar2017} (details on loss training and derivation) \cite{shen2014latent} or item embedding (top-k items retrieval using cosine distance) \cite{tan2016improved}, OHE item - masked (negative sampling) categorical cross-entropy with softmax \cite{hidasi2016} or Importance Sampling (Livro de DL - 12.4.3.3) with a  softmax + ranking-max loss function TOP1-max, BPR-max and additional negative samples (besides the ones in the mini-batch) \cite{hidasi2017} or Bayesian Personalized Ranking (BPR) \cite{liu2016context} \cite{rendle2009bpr}. More on softmax and Hierarquical Softmax / negative sampling: http://ruder.io/word-embeddings-softmax/
	\item Global effects: Take into account breaking news and seasonality (which may change the user reading behaviour across different news categories) \cite{epure2017recommending}. Logistic loss over the difference between the similarities of a clicked and negative item with the context item (upper bound the pairwise loss) \cite{gao2014modeling}.
	\item Multi-modal: Learn representations of both text and image?  \cite{hidasi2016parallel}
\end{itemize}

After an RNN, use attention weighted outputs instead of the last RNN hidden state, as in ... %http://smerity.com/articles/2016/google_nmt_arch.html


% Multi-label classification in Tensorflow: https://towardsdatascience.com/multi-label-image-classification-with-inception-net-cbb2ee538e30
%https://stackoverflow.com/questions/35400065/multilabel-text-classification-using-tensorflow




\subsubsection{Other inspirations from recent research on Deep NLP}
Highlights of EMNLP 2017: Exciting datasets, return of the clusters, and more...
http://ruder.io/highlights-emnlp-2017/index.html

...
Pinter et al. propose an approach for generating OOV word embeddings by training a character-based BiLSTM to generate embeddings that are close to pre-trained ones. This approach is promising as it provides us with a more sophisticated way to deal with out-of-vocabulary words than replacing them with an token.
http://aclweb.org/anthology/D/D17/D17-1010.pdf

Herbelot and Baroni slightly modify word2vec to allow it to learn embeddings for OOV words from few data.
http://aclweb.org/anthology/D/D17/D17-1030.pdf

Rosin et al. propose a model for analyzing when two words relate to each other over time.
http://aclweb.org/anthology/D/D17/D17-1122.pdf

Kutuzov et al. propose another model that analyzes how two words relate to each other over time.
http://aclweb.org/anthology/D/D17/D17-1194.pdf

Hasan and Curry improve the performance of word embeddings on word similarity tasks by re-embedding them in a manifold.
http://aclweb.org/anthology/D/D17/D17-1033.pdf
...


\subsubsection{Quasi-recurrent architecture} \cite{bradbury2016quasi}
Recurrent neural networks are a powerful tool for modeling sequential data, but the dependence of each timestep's computation on the previous timestep's output limits parallelism and makes RNNs unwieldy for very long sequences. We introduce quasi-recurrent neural networks (QRNNs), an approach to neural sequence modeling that alternates convolutional layers, which apply in parallel across timesteps, and a minimalist recurrent pooling function that applies in parallel across channels. Despite lacking trainable recurrent layers, stacked QRNNs have better predictive accuracy than stacked LSTMs of the same hidden size. Due to their increased parallelism, they are up to 16 times faster at train and test time. Experiments on language modeling, sentiment classification, and character-level neural machine translation demonstrate these advantages and underline the viability of QRNNs as a basic building block for a variety of sequence tasks.

%https://cdn.oreillystatic.com/en/assets/1/event/272/Backing%20off%20toward%20simplicity_%20Understanding%20the%20limits%20of%20deep%20learning%20Presentation.pdf
%https://einstein.ai/research/new-neural-network-building-block-allows-faster-and-more-accurate-text-understanding
%http://web.stanford.edu/class/cs224n/lectures/cs224n-2017-lecture9.pdf (end of lecture)

%Code PyTorch: https://github.com/salesforce/pytorch-qrnn

\subsubsection{Strongly-Typed Recurrent Neural Networks} \cite{balduzzi2016strongly}
Recurrent neural networks are increasing popular models for sequential learning. Unfortunately, although the most effective RNN architectures are perhaps excessively complicated, extensive searches have not found simpler alternatives. This paper imports ideas from physics and functional programming into RNN design to provide guiding principles. From physics, we introduce type constraints, analogous to the constraints that forbids adding meters to seconds. From functional programming, we require that strongly-typed architectures factorize into stateless learnware and state-dependent firmware, reducing the impact of side-effects. The features learned by strongly-typed nets have a simple semantic interpretation via dynamic average-pooling on one-dimensional convolutions. We also show that strongly-typed gradients are better behaved than in classical architectures, and characterize the representational power of strongly-typed nets. Finally, experiments show that, despite being more constrained, strongly-typed architectures achieve lower training and comparable generalization error to classical architectures.


\subsubsection{Pointer Sentinel Mixture Models} \cite{merity2016pointer}

Recent neural network sequence models with softmax classifiers have achieved their best language modeling performance only with very large hidden states and large vocabularies. Even
then they struggle to predict rare or unseen words even if the context makes the prediction unambiguous. We introduce the pointer sentinel mixture architecture for neural sequence models which has the ability to either reproduce a word from the recent context or produce a word from a standard softmax classifier. Our pointer sentinel LSTM model achieves state of the art language modeling performance on the Penn Treebank (70.9 perplexity) while using far fewer parameters than a standard softmax LSTM. In order to evaluate how well language models can exploit longer contexts and deal with more realistic vocabularies and larger corpora we also introduce the freely available WikiText corpus.
...

Attention-based pointer mechanisms were introduced in Vinyals et al. (2015) where the pointer network is able to select elements from the input as output. While pointer networks improve performance on rare words and long-term dependencies they are unable to select words that do not exist in the input.
...

\subsubsection{Tying Word Vectors and Word Classifiers: A Loss Framework for Language Modeling} \cite{inan2016tying}

Recurrent neural networks have been very successful at predicting sequences of words in tasks such as language modeling. However, all such models are based on the conventional classification framework, where the model is trained against one-hot targets, and each word is represented both as an input and as an output in isolation. This causes inefficiencies in learning both in terms of utilizing all of the information and in terms of the number of parameters needed to train. We introduce a novel theoretical framework that facilitates better learning in language modeling, and show that our framework leads to tying together the input embedding and the output projection matrices, greatly reducing the number of trainable variables. Our framework leads to state of the art performance on the Penn Treebank with a variety of network models.


%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Large Output Vocabularies}
Full softmax x Balanced Class Factorization x Balanced Tree Factorization x NCE / IS x Hierarchical Softmax
A Scalable hierarquical distributed language model. Mnih and Hinton, NIPS 09
Efficient softmax approximation for GPUs. Grave et al. arXiv, 2016
%https://github.com/oxford-cs-deepnlp-2017/lectures/blob/master/Lecture%204%20-%20Language%20Modelling%20and%20RNNs%20Part%202.pdf

%TODO: Pesquisar sobre Time-varying RNN \& Hierarchical Multiscale RNN



\section{Evaluation}
Describe evaluation across time \cite{beel2017s}


\section{Source codes}


%Code: https://github.com/hexiangnan/neural_collaborative_filtering


\subsection{TransNets: Learning to Transform for Recommendation}
Tensorflow code here!: 
https://github.com/rosecatherinek/TransNets

\subsection{Inter-Session Modeling for Session-Based Recommendation}
\cite{ruocco2017inter}: 
Tensorflow code available here (master thesis): 
%https://github.com/olesls/master_thesis


\subsection{3D Convolutional Networks for Session-based Recommendation with Content Features}
Tensorflow. Sent by e-mail


\subsection{Neural collaborative filtering}
\cite{he2017} : 
Keras
%https://github.com/hexiangnan/neural_collaborative_filtering

\subsection{Recurrent Neural Networks with Top-k Gains for Session-based Recommendations}
Theano
%https://github.com/hidasib/GRU4Rec

\subsection{Personalizing Session-based Recommendations with Hierarchical Recurrent Neural Networks}
\cite{quadrana2017personalizing}: (Theano) in 
%https://github.com/mquad/hgru4rec

\subsection{Context-Aware Sequential Recommendation}
Code available in (Pure Python): 
%http://qiangliucasia.github.io/homepage/files/CARNNcode.zip

\subsection{What to Do Next: Modeling User Behaviors by Time-LSTM}
Theano               
%https://github.com/DarryO/time_lstm
                     
\subsection{CF-NADE - A Neural Autoregressive Approach to Collaborative Filtering}
Theano               
%https://github.com/Ian09/CF-NADE	
                     
                     
\subsection{Attention-Based Convolutional Neural Network}
Tensorflow           
%TODO: Evaluate attention mechanism layer before and after convolution
%See code and paper in https://github.com/galsang/ABCNN
                     
%Deep Text Multi-lavel Text Classifiers in Tensorflow:https://github.com/brightmart/text_classification
%specially  Hierarchical Attention Network(HAN) (Bi-GRU + Attention)

\subsection{Benchmarks}
BPR-MF - theano-bpr:
%https://github.com/bbc/theano-bpr

CDAE - Collaborative Denoising Auto-Encoders
for Top-N Recommender Systems (C++)
%https://github.com/jasonyaw/CDAE

\subsection{Tools}
Embed.ly
%http://embed.ly/docs/explore/extract


Glove: https://nlp.stanford.edu/projects/glove/
%Word2Vec: https://code.google.com/archive/p/word2vec/

Embeddings:
German Embeddings (Word2Vec): http://devmount.github.io/GermanWordEmbeddings/
https://www.quora.com/Where-can-I-find-pre-trained-models-of-word2vec-and-sentence2vec-trained-on-Wikipedia-or-other-large-text-corpus
http://ahogrammer.com/2017/01/20/the-list-of-pretrained-word-embeddings/
https://github.com/Hironsan/awesome-embedding-models
%http://www.cs.cmu.edu/~afm/projects/multilingual_embeddings.html
https://news.ycombinator.com/item?id=13771292
https://github.com/Kyubyong/wordvectors

Tensorflow
%https://www.tensorflow.org/programmers_guide/embedding
https://www.tensorflow.org/tutorials/word2vec
https://www.tensorflow.org/tutorials/recurrent
%https://www.tensorflow.org/tutorials/deep_cnn

From [Learning Distributed Representations from Reviews for
Collaborative Filtering]
We preprocess reviews only by tokenizing
them using a script from Moses 6 , after which we build a
vocabulary of 5000 most frequent words.
https://github.com/moses-smt/mosesdecoder/

OpenRec - From "Immersive Recommendation" presentation
https://github.com/ylongqi/OpenRec

QRNN 
- PyTorch
https://github.com/salesforce/pytorch-qrnn
-TensorFlow
%- https://github.com/icoxfog417/tensorflow_qrnn
- https://github.com/santi-pdp/quasi-rnn
- https://github.com/shoarora/tf-qrnn


Pairwise Ranking Losses
https://stackoverflow.com/questions/40330775/compute-efficiently-a-pairwise-ranking-loss-function-in-tensorflow
https://github.com/fchollet/keras/issues/4861
%- https://www.tensorflow.org/api_guides/python/contrib.losses

XCLiMF
https://github.com/timotta/xclimf
http://programandosemcafeina.blogspot.com.br/




%TODO: Inspiration on How to model popularity, recency and recommendatinos diversity \cite{li2011scene}


%TODO: Inspiration for loss function design (matrix factorization), Weighted Approximate-Rank Pairwise (WARP), and SGD algorithm. It also used a simulated online evaluation \cite{diez2016}

%TODO: Methods for Implicit Feedback Ranking: Bayesian Personalized Ranking (BPR) and Weighted Approximate-Rank Pairwise (WARP). Warp++ \cite{shashkin2017learning}

Recommendation task can be naturally posed as a ranking problem where for each user we are trying to rank positive items higher than negative ones. In implicit setting pairwise learning methods like Bayesian Personalized Ranking (BPR) [13] assume that all unobserved user-item interactions are negative and minimize ranking loss by triplets (user, positive item, negative item) \cite{shashkin2017learning}. 
To reduce computational complexity negative items are sampled uniformly. It has been shown that more sophisticated adaptive sampling procedures[12, 14] perform more informative parameter updates and improve calculable performance metrics. In the WARP algorithm the loss function is similar to hinge loss weighted by the rank of positive item. Only triplets that violate the desired order are used to update model parameters \cite{shashkin2017learning}.

%TODO: example on Online Loss Optimization \cite{shashkin2017learning}



==> Cap5/cap5-notes.tex <==


%TODO: In \cite{das2007} evaluation (Google) they select the top 5000 users (with more clicks), ignoring the top 1000, since they have an unusually large number of clicks and are suspected to be bots as opposed to real humans

%TODO: Interesting analysis from Google News on how users topics change over time \cite{liu2010personalized}. See click distribution distance metrics. May be useful for an EDA on Chap 5.

%TODO: Reference on hypothesis testing using chi-square \cite{epure2017recommending}


%In Today-Module on Yahoo! Front Page, 40\% of clickers are new clickers with no historical clicks, 82\% of clickers have less or equal to 5 historical clicks, 92\% of clickers have no more than 10 historical clicks \cite{chu2009personalized}.


%TODO: See analysis of time elapsed between interactions and also clicks within X time after publishing \cite{shashkin2017learning}
Figure 1 illustrates previously used notion of session as well as seasonality. We assume that the first two spikes (around one second and one minute marks) indicate whether user skipped content or interacted with it. The rightmost density increase demonstrates the time intervals between sessions (note the daily and weekly visitors).
Unfortunately, the value used to identify the user is not very reliable for the majority of users, it is not same across different devices or browsers. \cite{shashkin2017learning}




\section{Datasets}

\subsection{CI\&T DeskDrop - Articles sharing and reading}

Domain: Web articles sharing in a corporate social network 
 
User identification: always logged  

User interactions: Views, likes, comments, follow, bookmark  

\begin{itemize}
	\item Item: Url, title, text, creation data, lang, tags? (may leverage the boards for this) 
	\item User visit: user, session, timestamp, geo (state / country), user-agent
\end{itemize}


\subsection{CLEF NewsReel - News reading (German)}

Domain: News reading

User identification: Device cookies

User interactions: Clicks

Idea: Use this dataset to classify news and get better news categories for CLEF: https://www.kaggle.com/uciml/news-aggregator-dataset
https://www.kaggle.com/uciml/news-aggregator-dataset

References:
- Shedding Light on a Living Lab: The CLEF NEWSREEL Open Recommendation Platform \cite{brodt2014shedding}
- CLEF 2017 NewsREEL Overview - Offline and Online Evaluation of Stream-based News Recommender Systems2017.pdf \cite{kille2017clef}


The News Recommendation Challenge. The CLEF NewsREEL
challenge allows researchers to analyze news recommender algorithms
based on real-life data both online and offline. The task
in the challenge consists of providing recommendation for popular
German online news portals. The recommendations are typically
placed below a news article in a box labeled "Also interesting" \cite{lommatzsch2017incorporating}

[12] Frank Hopfgartner, Torben Brodt, Jonas Seiler, Benjamin Kille, Andreas Lom-
matzsch, Martha Larson, Roberto Turrin, and András Serény. 2016. Benchmarking
News Recommendations: The CLEF NewsREEL Use Case. SIGIR Forum 49, 2 (Jan.
2016), 129–136. https://doi.org/10.1145/2888422.2888443


PLISTA is the leading recommendation and advertising network in the German-speaking market. PLISTA collects user interactions from websites and provides recommendations that are integrated into the website. The cooperation allows us to perform an online as well as an offline evaluation, testing our algorithms in a real-world environment \cite{lommatzsch2014real}.



The disadvantage of the near-to-online evaluation is that the evaluation is biased towards the popular algorithms: Since positive feedback is always the result of a recommendation, the algorithms selected for placing the results on a news article web page define what set of articles the user can click on. That means, that the
algorithms used by other teams in the contest, influence the measure near-to-online performance. Due to the fact, there is nothing known about the algorithms used by other teams, the feedback (caused by recommendations from other teams) helps exploring new aspects. About 95\% of the feedback messages are based on recommendations from other teams. \cite{lommatzsch2014real}


\begin{itemize}
	\item Item: Url, title, text, domain, image, creation date
	\item User visit: user, date time, geo, category, publisher, time to action.
	Ps. Sessions might be inferred by manually split sessions according to \ref{epure2017recommending}
\end{itemize}


\subsection{Life.ru - Russian}

The data is collected from popular Russian news website 1 . In addition to big (30 millions users by 140 thousands articles) and sparse (440 millions nonzero values) binary matrix the dataset also contains time for each interaction. Many users appear only once and even without taking them into account 49.7\% of remaining users interact with the website only within 24 hours interval. We share this dataset 2 to make our results reproducible \cite{shashkin2017learning}.

\subsection{Adressa dataset - Norwegian}
Gulla, Jon Atle, et al. "The Adressa dataset for news recommendation." Proceedings of the
International Conference on Web Intelligence. ACM, 2017.
http://delivery.acm.org/10.1145/3110000/3109436/p1042-gulla.pdf

References: 
The Adressa Dataset for News Recommendation2017.pdf

If full text is not available via APIs, use Embed.ly
%http://embed.ly/docs/explore/extract


%\subsection{Model architecture}

%\subsubsection{Objective function}

%Traditional matrix factorization based recommendation methods take the sum-of-squares of factorization errors as the objective function, which can be regarded as point-wise methods. Recently, some pair-wise methods, such as BPRMF \cite{gantner2012personalized} and Weighted BPRMF (WBPMF) \cite{rendle2009bpr}, are proposed, in which the pair-wise comparison error is minimized. List-wise methods are also proposed, such as ListPMF \cite{liu2014list} and QMF \cite{shi2012climf}. In these methods, the recommended item list is regarded as a whole instance, and the log-posterior over the recommended item list with the observed preference orders is maximized \cite{wu2016recurrent}. 


\section{Evaluation}
Describe evaluation across time \cite{beel2017s}


\section{Source codes}

%A library for efficient similarity search and clustering of dense vectors. - https://github.com/facebookresearch/faiss

%Introduction to LSTMs with TensorFlow: https://www.oreilly.com/ideas/introduction-to-lstms-with-tensorflow?imm_mid=0fa998&cmp=em-data-na-na-newsltr_ai_20180122


Tensorflow Text Classification examples!
%https://github.com/brightmart/text_classification

%Code: https://github.com/hexiangnan/neural_collaborative_filtering


\subsection{TransNets: Learning to Transform for Recommendation}
Tensorflow code here!: 
https://github.com/rosecatherinek/TransNets

\subsection{Inter-Session Modeling for Session-Based Recommendation}
\cite{ruocco2017inter}: 
Tensorflow code available here (master thesis): 
%https://github.com/olesls/master_thesis


\subsection{3D Convolutional Networks for Session-based Recommendation with Content Features}
Tensorflow. Sent by e-mail


\subsection{Neural collaborative filtering}
\cite{he2017} : 
Keras
%https://github.com/hexiangnan/neural_collaborative_filtering

\subsection{Recurrent Neural Networks with Top-k Gains for Session-based Recommendations}
Theano
%https://github.com/hidasib/GRU4Rec

\subsection{Personalizing Session-based Recommendations with Hierarchical Recurrent Neural Networks}
\cite{quadrana2017personalizing}: (Theano) in 
%https://github.com/mquad/hgru4rec

\subsection{Context-Aware Sequential Recommendation}
Code available in (Pure Python): 
%http://qiangliucasia.github.io/homepage/files/CARNNcode.zip

\subsection{What to Do Next: Modeling User Behaviors by Time-LSTM}
Theano               
%https://github.com/DarryO/time_lstm
                     
\subsection{CF-NADE - A Neural Autoregressive Approach to Collaborative Filtering}
Theano               
%https://github.com/Ian09/CF-NADE	
                     
                     
\subsection{Attention-Based Convolutional Neural Network}
Tensorflow           
%TODO: Evaluate attention mechanism layer before and after convolution
%See code and paper in https://github.com/galsang/ABCNN
                     
%Deep Text Multi-lavel Text Classifiers in Tensorflow:https://github.com/brightmart/text_classification
%specially  Hierarchical Attention Network(HAN) (Bi-GRU + Attention)

%Best paper runner up RecSys 2017: Translation-based Recommendation
%Models next-best actions
%http://cseweb.ucsd.edu/~jmcauley/pdfs/recsys17.pdf


\subsection{Benchmarks}
BPR-MF - theano-bpr:
%https://github.com/bbc/theano-bpr

CDAE - Collaborative Denoising Auto-Encoders
for Top-N Recommender Systems (C++)
%https://github.com/jasonyaw/CDAE

\subsection{Tools}
Embed.ly
%http://embed.ly/docs/explore/extract


Glove: https://nlp.stanford.edu/projects/glove/
%Word2Vec: https://code.google.com/archive/p/word2vec/

Embeddings:
German Embeddings (Word2Vec): http://devmount.github.io/GermanWordEmbeddings/
https://www.quora.com/Where-can-I-find-pre-trained-models-of-word2vec-and-sentence2vec-trained-on-Wikipedia-or-other-large-text-corpus
http://ahogrammer.com/2017/01/20/the-list-of-pretrained-word-embeddings/
https://github.com/Hironsan/awesome-embedding-models
%http://www.cs.cmu.edu/~afm/projects/multilingual_embeddings.html
https://news.ycombinator.com/item?id=13771292
https://github.com/Kyubyong/wordvectors

Tensorflow
%https://www.tensorflow.org/programmers_guide/embedding
https://www.tensorflow.org/tutorials/word2vec
https://www.tensorflow.org/tutorials/recurrent
%https://www.tensorflow.org/tutorials/deep_cnn

From [Learning Distributed Representations from Reviews for
Collaborative Filtering]
We preprocess reviews only by tokenizing
them using a script from Moses 6 , after which we build a
vocabulary of 5000 most frequent words.
https://github.com/moses-smt/mosesdecoder/

OpenRec - From "Immersive Recommendation" presentation
https://github.com/ylongqi/OpenRec

QRNN 
- PyTorch
https://github.com/salesforce/pytorch-qrnn
-TensorFlow
%- https://github.com/icoxfog417/tensorflow_qrnn
- https://github.com/santi-pdp/quasi-rnn
- https://github.com/shoarora/tf-qrnn


Pairwise Ranking Losses
https://stackoverflow.com/questions/40330775/compute-efficiently-a-pairwise-ranking-loss-function-in-tensorflow
https://github.com/fchollet/keras/issues/4861
%- https://www.tensorflow.org/api_guides/python/contrib.losses

XCLiMF
https://github.com/timotta/xclimf
http://programandosemcafeina.blogspot.com.br/


https://www.kaggle.com/c/mercari-price-suggestion-challenge/discussion/50256
NLP researchers need to work with custom CUDA code (e.g. http://riejohnson.com/cnn\_download.html), and this is holding back progress in many ways. 

FastText (MLP with n-grams)
https://martinbel.github.io/fast-text.html
https://arxiv.org/pdf/1607.01759v3.pdf



%See RNN regularization: Variational Dropout \cite{gal2016theoretically} / zoneout \cite{krueger2016zoneout}







%TODO: Concact Bibblio

---------- Forwarded message ---------
From: Daan Odijk <daan@blendle.com>
Date: sex, 8 de dez de 2017 às 08:28
Subject: Re: [research] ICT with Industry 2017 dataset
To: Gabriel de Souza Pereira Moreira <gspmoreira@gmail.com>


Hi Gabriel,

Thanks for your interest in Blendle and the workshop. We ended up working with a dataset of news articles, without any user behavior. I don't think this would really help with your research. 

Do you know the London-based company Bibblio? You could try to contact Robbert (https://twitter.com/rvanderpluijm) for a collaboration. They recommend news for publishers and are keen on learning more about deep learning.

Best of luck with your PhD.

  Daan
  
%ttps://twitter.com/rvanderpluijm
%https://twitter.com/Bibblio_org
%http://www.bibblio.org/
  
  
  
  
  %%%%% Previous final of Chapter 5 at Qualifying time
  
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  
  
  \subsection{Evaluation}

This implementation of the CNN-based architecture instantiation of the ACR module was evaluated on CLEF-NewsREEL dataset, described in detail in Section \ref{sec:news-dataset}. 

The evaluation goal was to predict the news article category based on the article's textual content and on side metadata - news publisher, in this case. 

\subsubsection{Dataset}

The CLEF-NewsREEL dataset, described in Section \ref{sec:clef-newsreel}, contains 6512 news articles with valid categories. An article content consists of its title, a 'kicker' -- text that usually appear above the headline in news portals -- and a short description. The median number of words by article is 36, and the largest article has 75 words.

Articles are distributed in 235 categories, from 4 different publishers. Only articles with a valid category (6512 of those) were used in this evaluation.

In Figure \ref{figure:cat-distribution}, it can be seen the long-tail distribution of the number of articles by categories. That is a common scenario in a news portal, as popular topics like sports and entertainment have usually more articles published.

\begin{figure}[h]
	\centering
	\includegraphics[width=15cm]{Cap5/cat_distribution.png}	\caption{News articles by categories distribution}
	\label{figure:cat-distribution}
\end{figure}


\subsubsection{Pre-training of word embeddings}

As the target articles are in German language, the first step was to train German word embeddings. The Gensim framework \cite{rehurek_lrec2010_gensim} and a toolkit to train German Word Embeddings \cite{germanwordembeddingstoolkit} were used to  train Word2Vec models \cite{mikolov2013distributed} in an unsupervised way. 

The large training corpus was composed of a dump of the German Wikipedia \cite{wikipedia}, with more than 2 million articles, and a dataset of 34 million news headlines, crawled from news portals \cite{bojar2014findings}.

Word2Vec models were trained by using Skip-gram and Hierarchical Softmax to produce word embeddings with 200 dimensions. Two Word2Vec models were trained for evaluation -- the first representing all words that occur less than 5 times in the whole corpus, configured with a window size of 7 words (Word2Vec-A), and the second filtering out words that occur less than 10 times, as well as common German stopwords and punctuation, configured with a window size of 5 words (Word2Vec-B).

After training, Word2Vec-A model had a vocabulary of 2,047,462 words. About 97\% of the (non-unique) words of CLEF-NewsREEL dataset were present in the Word2Vec model -- a total of 40149 unique words.

The Word2Vec-B model had a vocabulary of 1,163,190 words. Its words coverage on CLEF-NewsREEL dataset was 55\%, which represent 38879 unique words.

\subsubsection{Baseline algorithms}

A set of traditional algorithms were used as baselines for the task of text classification: Naive Bayes \cite{manning20introduction}, Random Forests \cite{forests2001leo}, and Extra Trees \cite{geurts2006extremely}.

As the input for those algorithms, the popular TF-IDF method \cite{ramos2003using}, from Information Retrieval, was used to vectorize news' textual content. The TF-IDF reflects how important is each word to a document in a collection. This method is widely used in search and text classification tasks.

%TODO: TF-IDF equations


\subsubsection{Input pre-processing}

Initially, it was necessary to preprocess the textual content of the 6512 articles from CLEF-NewsREEL dataset.

For the baseline algorithms, the TF-IDF method was used to produce a vector for each article, which dimension was a fixed vocabulary of the 5000 more frequent words in the corpus. 

After the TF-IDF model training, vectors were concatenated with a news metadata -- the article publisher -- represented as a one-hot encoded categorical feature.

For the CNN-based implementation of the ACR module, each word was converted to the index number of the corresponding word embedding. Out-of-vocabulary words were replaced by the index of the special '<UNK>' token. 

The articles vectors length was fixed to the maximum number words (with corresponding word embeddings) of any article -- 68 in this case. Shorter articles were padded with the index of the special '<PAD>' token. The embeddings vectors for '<UNK>' and '<PAD>' special tokens were randomly initialized and fixed.

The one-hot encoded publisher was also used as input for the CNN-based model, joined with the convolution layers output.

\subsubsection{Classification Results}

Models were compared by the Accuracy metric, which is the percentage of news articles for which their categories were correctly classified. 

The dataset samples were split in 80\% for training, 10\% for validation and 10\% for test. The hyperparameters of the algorithms were tuned based on accuracy on validation set. 

The evaluation results are presented in Figure \ref{figure:news_category_classification}, where  classification accuracy is reported for test set.

\begin{figure}[h]
	\centering
	\includegraphics[width=16cm]{Cap5/news_category_classification.png}	
	\caption{Models accuracy on news category classification}
	\label{figure:news_category_classification}
\end{figure}


It can be observed that baseline models had a similar accuracy, probably limited because of its input textual representation (TF-IDF).

The CNN-based models have presented a significantly better accuracy. That result highlights how effective was the usage of pre-trained word embeddings and of a CNN architecture for text classification. 

From the difference of accuracy between the two CNN models using Word2Vec-A embeddings, it can be seen that news metadata features (publisher) may really add predictive power to the network.

The best accuracy was obtained by the CNN model, by using Word2Vec-B embeddings as inputs. This finding contradicted the initial research  expectation, because this version of the Word2Vec model did not include stopwords and punctuation, and had only 55\% of its words represented as embeddings. 

From this experiment, it appears that CNNs were not able to leverage stopwords and punctuation for a better representation of the text. The current belief is that an RNN-based instantiation of the ACR module might be benefit from such additional tokens. RNN architectures processes text in sequence, thus stopwords and punctuation may be important for better 'understanding' of the sentences.

\subsubsection{The Article Content Embeddings Evaluation}

Text classification is not the main objective of the ACR module. It is only a side task, used to produce Article Content Embeddings that really represents the content of the article.

To evaluate the quality of the Article Content Embeddings, it was used a probabilistic dimensionality reduction technique named t-Distributed Stochastic Neighbor Embedding (t-SNE) \cite{maaten2008visualizing}, which usually produces better embedding visualizations than Principal Component Analysis (PCA). In Figure \ref{figure:t-sne_article_embeddings_merged}, it is presented a t-SNE visualization of Article Content Embeddings, sampled from articles of the top 15 categories within the test set  \ref{figure:t-sne_article_embeddings_merged}. 

\begin{figure}[h]
	\centering
	\includegraphics[width=16cm]{Cap5/clef_newsreel_testset_517_top15cat_embeddings_scatterplot_merged.png}	
	\caption{Article Content Embeddings (t-SNE) from the CLEF-NewsREEL test set sampled articles. Colors in the left and right scatter plots represent publishers and categories, respectively.}
	\label{figure:t-sne_article_embeddings_merged}
\end{figure}

The left scatter plot represent news articles colored by their publishers. Clearly, the learned article embeddings can be easy separated by publisher. That is not surprising, as the publisher was used as an input feature.

The right scatter plot presents articles colored by their category, which was used as the training output of the ACR module. It is possible to observe that articles of some categories are well clustered, while for other categories they are a little spread. This indicates that, to some extent, the ACR module was able to produce article embeddings that maximize similarity within their category and minimize similarity with articles from other categories.

For a qualitative evaluation of Article Content Embeddings, articles similarities were computed, by using the cosine similarity (Equation \ref{eq:cosine_sim}). Table \ref{tab:similar-embeddings-sports} presents, in its first line, the content of a random article from about "sports" (German language), followed by the four most similar articles. Table \ref{tab:similar-embeddings-berlin} does the same for an article about "Berlin" city. By the content of the articles, it can be observed that they are really related. 

\begin{table}[htbp]
\centering
\caption{Similar articles about "sports"}
\label{tab:similar-embeddings-sports}
\begin{tabular}{|p{13cm}|c|}
\hline
\textbf{Article Content (Title | Kicker | Description)} & \textbf{Similarity} \\ \hline

Kommentar: Generation Mut | Kommentar von Alexander W\"{o}lffing zur Handball-Nationalmannschaft bei der EM | Der offensive Ansatz des Deutschen Handball-Bundes um Bob Hanning zahlt sich aus. Alexander W\"{o}lffing, stellvertretender Chefredakteur und Leiter Sports bei SPORT1,  kommentiert.                                      & -                      \\ \hline \hline

"Seahawks werden Brady bearbeiten" | NFL-Legende Hines Ward analysiert den Super Bowl | Hines Ward favorisiert Seattle. Der fr\"{u}here MVP des Endspiels sieht aber Vollmer und Co. sowie einen X-Faktor als Chance der Patriots. F\"{u}r SPORT1 analysiert er den Super Bowl.
& 0.970                      \\ \hline

Bald kein "Hack-a-Drummond" mehr? | Foul als taktisches Mittel: NBA will "hack-a-player"-Regel \"{a}nder | Andre Drummond und alle schlechten Freiwerfer in der NBA wird es freuen: Die Liga will Fouls als taktisches Mittel anders bestrafen, um den Sport nicht kaputt zu machen.
& 0.964                      \\ \hline
Nummer 2: Leno findet sich damit ab | Bernd Leno spricht im SPORT1-Interview \"{u}ber Manuel Neuer | Bayer Leverkusens Bernd Leno nimmt bei SPORT1 Stellung zur Torh\"{u}ter-Situation im DFB-Team sowie Vorbild Manuel Neuer - und spricht auch \"{u}ber Fehler und Frust.                                                       & 0.962                      \\ \hline

"Es gibt eine Strafe gegen Schmidt" | Nach dem Eklat um Leverkusens Trainer Roger Schmidt spricht DFB-Chefankl\"{a}ger bei SPORT1 | Der historische Eklat um Leverkusens Coach Roger Schmidt erhitzt Fu\ss{}ball-Deutschland. Es wird eine Strafe f\"{u}r Schmidt geben. Bei SPORT1 spricht jetzt der DFB-Chefankl\"{a}ger.
& 0.959                     \\ \hline

\end{tabular}
\end{table}





\begin{table}[htbp]
\centering
\caption{Similar articles about "Berlin"}
\label{tab:similar-embeddings-berlin}
\begin{tabular}{|p{13cm}|c|}
\hline
\textbf{Article Content (Title | Kicker | Description)} & \textbf{Similarity} \\ \hline

Jetzt fahr'n wir \"{u}bern See | Stadtsafari - Sommerliche Entdeckertouren in Berlin (4) | Lust auf eine Radtour links und rechts der Havel? Von Wannsee nach Kladow und Sacrow bis nach Babelsberg? Machen Sie einen Ausflug \"{u}bers Wasser zu Schl\"{o}ssern und Parks. Denn gottseidank gibt's ja F\"{a}hren... & -                      \\ \hline \hline

Mauer-Reste in Berlin: Die Stadt ist ein hartes Pflaster | Wo steht sie heute noch? | Von Kladow bis Kreuzberg, vom Mauerpark bis zum Europacenter: Wo ist im Jubil\"{a}umsjahr 2014 noch ein St\"{u}ck Berliner Mauer zu finden?
& 0.943                      \\ \hline

Hauptbahnhof und Co.: Die Unvollendeten | Bahnstationen in Berlin | Am Hauptbahnhof fehlen Zubringer, am S\"{u}dkreuz gibt es weiter keine Parkh\"{a}user und am Gesundbrunnen kommt das Empfangsgeb\"{a}ude mit reichlich Versp\"{a}tung: Sieben Jahre nach der Er\"{o}ffnung liegt bei Berlins gro\ss{}en Bahnstationen noch so einiges im Argen.
& 0.937                      \\ \hline

Hundert Jahre Wilmersdorfer Eva-Lichtspiele | Berliner Kino-Legende | Ganz lupenrein ist das Datum ja nicht. Aber trotzdem wird an der Wilmersdorfer Blissestra\ss{}e gro\ss{} gefeiert. Denn seit 1913 gibt es hier ein Kino - die legend\"{a}ren ,,Eva-Lichtspiele\textquotedblleft{}. F\"{u}r das Jubil\"{a}um hat sich der Chef etwas Besonderes ausgedacht.
& 0.927                      \\ \hline

Neue Ideen f\"{u}r Hochhaus nahe Bahnhof Zoo | Berlin-Charlottenburg | Das Gel\"{a}nde zwischen Landwehrkanal und Bahnhof Zoo liegt ziemlich brach. Stararchitekt Jan Kleihues m\"{o}chte das Viertel entwickeln. Mit Studenten hat er nun neue Pl\"{a}ne entwickelt.
& 0.917                     \\ \hline

\end{tabular}
\end{table}


In Figure \ref{figure:t-sne_article_similar_embeddings}, the "sports" related articles from Table \ref{tab:similar-embeddings-sports} are highlighted with red circles, and the articles about "Berlin" from Table \ref{tab:similar-embeddings-berlin} are highlighted by black circles. Visually, it can be seen that t-SNE dimensionality reduction preserves similarity properties from the original embeddings.

\begin{figure}[h]
	\centering
	\includegraphics[width=16cm]{Cap5/clef_newsreel_testset_517_top15cat_categories_embeddings_scatterplot_docs_similarity_highlighted.png}	
	\caption{Article Content Embeddings (t-SNE) from CLEF-NewsREEL test set sampled articles. Dot colors represent categories, and circled dots represent similar articles}
	\label{figure:t-sne_article_similar_embeddings}
\end{figure}



\subsection{Discussion of the results}

In Chapter 1, the first stated hypothesis (HY1) was that Deep Learning could be used to learn  representations for articles' textual content that are effective news recommendation.

By the instantiation, implementation and evaluation of the ACR module, it was possible to observe that a Deep Learning architecture -- the CNN, in this case -- is able to learn article embeddings directly from  textual content. 

The learned article embeddings provided a much superior performance on the news category classification, when compared to other traditional baseline algorithms, by using statistical-based textual representation (e.g., TF-IDF). 

The similarity among article embeddings was successful in clustering together articles with related content. This is very important for the CHAMELEON Meta-Architecture, in which items are represented by the Article Content Embeddings instead of item IDs, to deal smoothly with the cold-start problem.

Although, it was not possible yet to test the HY1 hypothesis, for which the CHAMELEON recommendation effectiveness must be evaluated as, for that, it will be necessary the instantiation, implementation, and evaluation of the NAR module.


%\subsection{The NAR module evaluation}
%- Time-aware evaluation
%- Metrics (NDCG, MAP, MRR)

\section{News Datasets}
\label{sec:news-dataset}
For the CHAMELEON Meta-Architecture offline evaluation of News Recommendations, it was necessary to obtain some datasets of logged user interactions on news portals. Furthermore, as the proposed meta-architecture is a hybrid recommender system, the textual content of the articles was also required. Three news portals' datasets meeting these requirements were investigated and obtained to make the offline evaluation possible.

\subsection{The CLEF-NewsREEL dataset}
\label{sec:clef-newsreel}

The News REcommendation Evaluation Lab (NewsREEL) is a campaign-style challenge offered by CLEF \cite{ferro2014clef}, since 2014 \cite{hopfgartner2016benchmarking}. It provides an environment for researchers to analyze news recommender algorithms based on real-life data, both in online and offline evaluation settings. 

The NewsREEL Living Lab \cite{brodt2014shedding} challenge consists of providing real-time recommendations for real users of popular online news portals from German-speaking countries \cite{brodt2014shedding} \cite{kille2017clef}. For each recommendation request, a participant has to provide a list of up to six recommendations, in a time constraint of 100 milliseconds. The recommendations are typically placed below a news article in a box labeled "Also interesting" \cite{lommatzsch2017incorporating}. Participants' algorithms performance is evaluated, by using the  Click-Through Rate (CTR) metric. 

The CLEF-NewsREEL also offers a dataset for offline evaluation of news recommendation. It covers a period of four weeks, starting on February 1, 2016 \cite{kille2017clef}. It comprises some events like news articles publishing and user clicks on articles. 

The dataset contains about 1.5 million of clicks on more than 6 thousand articles, made by about 600 thousands of users. 

The dataset is very long-tailed in the number of interactions by users, as usual in news portals -- 75\% of users have visited at most two articles, during the whole month period.

The CLEF-NewsREEL dataset contains information about the published articles (e.g., URL, title, kicker, text, publisher, category, display image, creation date) and about user visits (e.g., user id, clicked article id, timestamp, geo-location, time-to-action). 
%s. Sessions might be inferred by manually split sessions according to \ref{epure2017recommending}

%Within NewsREEL, the infrastructure is provided by plista GmbH2 , a company that offers recommendation services for online publishers. Whenever a user requests an article from one of their customers’ web portals, plista recommends further articles that the user might be interested in. In NewsREEL, plista outsources a subset of this recommendation task to interested researchers via their Open Recommendation Platform (ORP) [3]. Once a user visits a news web page assigned to the NewsREEL challenge, a recommendation request is sent to a randomly selected team who registered with ORP. For each request, the team then has to provide a list of up to six recommendations. Providing recommendations to real users, a time constraint of 100ms is set for completing the recommendation request.


%PLISTA is the leading recommendation and advertising network in the German-speaking market. PLISTA collects user interactions from websites and provides recommendations that are integrated into the website. The cooperation allows us to perform an online as well as an offline evaluation, testing our algorithms in a real-world environment \cite{lommatzsch2014real}.

%The disadvantage of the near-to-online evaluation is that the evaluation is biased towards the popular algorithms: Since positive feedback is always the result of a recommendation, the algorithms selected for placing the results on a news article web page define what set of articles the user can click on. That means, that the algorithms used by other teams in the contest, influence the measure near-to-online performance. Due to the fact, there is nothing known about the algorithms used by other teams, the feedback (caused by recommendations from other teams) helps exploring new aspects. About 95\% of the feedback messages are based on recommendations from other teams. \cite{lommatzsch2014real}


\subsection{The Adressa dataset}

The Adressa dataset was prepared as part of the RecTech project on recommendation technology -- a 4.2 million Euro industry-led research project that was started in 2016 and was partly funded by the Research Council of Norway. The project owner was Adresseavisen  (with short form "Adressa") -- the largest newspaper in the Polaris Media news house, with around 140,000 daily readers \cite{gulla2017adressa}. 

The Adressa dataset covers three months of web traffic (from January 1 to March 31, 2017) on the \textit{www.adresseavisen.no} web site. All articles in the dataset are in Norwegian language, and the average article length is 518 words. Of the 15,514 readers in the dataset, 672 are registered subscribers \cite{gulla2017adressa}.
%TODO: Confirm stats for the 3-months dataset (those are statistics from the 1-week dataset)

For each user click, the dataset contains information about the article, user session, and context (e.g., clicked article id, title, author, URL, category, user id, city, region, country, and device operational system). The article's textual content can be extracted by crawling their URLs pages.

In that dataset, every session constitutes a new user ID. A particular reader will be associated with a new user ID, every time a new session is initiated or when using a different device \cite{gulla2017adressa}.

\subsection{The Life.ru dataset}

The Life.ru dataset was collected from a popular Russian news website and shared by \cite{shashkin2017learning}, to make reproducible their research on factorization models for news recommendations. 

The dataset covers all user interactions during a month, from March 12 to April 12, 2017. It contains 30 millions users interactions on 140 thousands articles. Daily, they have about 300 new published articles, 800 thousand unique visitors, and more than 2 million user interactions. About 86\% of articles views are within the first 24 hours after its publishing.

Many users appear only once in the dataset. Even ignoring such users, 49.7\% of remaining users interact with the website only within a 24 hours interval \cite{shashkin2017learning}.

The dataset contains logged user interactions on articles, with timestamps. Articles' title and subtitle are also available. Articles' full textual content may be crawled, by using the articles URLs. Unfortunately, this dataset does not include user contextual information like location and device.

%TODO: Add dataset distribution charts provided in the \cite{shashkin2017learning} presentation slides


\section{Research Current State and Next-Steps}

In Chapter 1, this author established the following requirements for this research.

\begin{itemize}
\item RRQ1 - Investigate state-of-art methods for news recommendations;
\item RRQ2 - Investigate state-of-art Deep Learning methods applied for recommender systems;
\item RRQ3 - Elaborate a Deep Learning meta-architecture for news recommendations;
\item RRQ4 - Implement and evaluate some instantiation of the proposed meta-architecture; and
\item RRQ5 - Test stated hypotheses based on evaluation results.
\end{itemize}

Up to now, the research requirements RRQ1, RRQ2, and RRQ3 were already fulfilled, as reported in Chapters 2, 3, and 4, respectively.

The RRQ4 is being currently addressed, as described in Chapter 5. A first architecture instantiation of the ACR module was proposed and implemented. It was evaluated, in terms of new metadata prediction accuracy. Article Metadata Embeddings were also projected and visualized, for a qualitative assessment of the relatedness of similar articles embeddings.

The next activities for accomplishing RRQ4 and RRQ5 are:

\begin{itemize}
\item To train word embeddings, by using a different method than Word2Vec, like GloVe, and also to evaluate the performance of the ACR module in news metadata prediction;
\item To elaborate an RNN-based instantiation of the ACR module, and also to implement and evaluate it in the TensorFlow;
\item To elaborate instantiations of the NAR module, and also to implement and evaluate them in the TensorFlow; and
\item To test stated research hypotheses, by using offline evaluation on three different news datasets.
\end{itemize}

If the CLEF-NewsREEL Living Lab is offered in the upcoming year (2018) or if a partnership can be established with a large news portal, it will be possible to conduct an online live evaluation of a CHAMELEON architecture instantiation with real users.
  
  
  
  

==> trash.tex <==
With the overwhelming information on the Internet and limitations of one-fit-all search engines, advanced tools are required to enable users to find the right information (Jawaheer, G., 2014).

Other methods commonly used for recommendation systems are bayesian inference, and case-based reasoning methods \cite{Smyth2007}. These methods consider the actual content or attributes of the items to be recommended instead of or in addition to user rating patterns. 



However, little attention has been paid to the application of the user model in recommender systems, particularly the variability and noise that are an intrinsic part of human behavior and activity \cite{jawaheer2014}. 


To enable recommender systems to suggest items that are useful to a particular user, it can be essential to understand the user and his or her interactions with the system \cite{jawaheer2014}.


Constructing user preference profiles is crucial for accurate predictions in recommendation systems. While traditional profiling is well understood, modern dynamic online recommendation services raise interesting challenges for user profiling. First, effectively representing user preferences in dynamic settings requires novel modeling techniques such as latent factorization. Second, for space and time efficiency, it might be infeasible to store all observed user profile signals, which requires resorting to streaming or sketching algorithms. Third, there are significant engineering architecture challenges to efficiently maintain user profiles for large-scale real-time recommendations (RecProfile workshop 2016).






The work that is most relevant to my research are \cite{wu2016}, \cite{he2017} and \cite{kumar2017}. 

In \cite{wu2016} a collaborative denoising autoencoder (CDAE) for CF with implicit feedback is presented. In contrast to the DAE-based CF \cite{strub2015}, CDAE additionally plugs a user node to the input of autoencoders for reconstructing the user's ratings. Although CDAE is a collaborative filtering model, it is solely based on item-item interaction.

In \cite{he2017}, authors have explored deep neural networks for recommender systems. They present a general framework named NCF, short for Neural Collaborative Filtering that replaces the inner product with a neural architecture that can learn an arbitrary function from the given data. It uses a multi-layer perceptron to learn the user-item interaction function. NCF is able to express and generalize matrix factorization. They then combine the linearity of matrix factorization and non-linearity of deep neural networks for modeling user-item latent structures. They call this model as NeuMF, short for Neural Matrix Factorization.


User profiling is an important step for solving the problem of personalized textual content recommendation. Traditional user profiling techniques often construct profiles of users based on static historical data accessed by users. However, due to the frequent updating of news repository, it is possible that a user's fine-grained reading preference would evolve over time while his/her long-term interest remains stable (LI, 2013). User profiles are temporal, and changes in a user's activity patterns are particularly useful for improved prediction and recommendation \cite{ahmed2011}.




A topic model is a generative model which include latent properties called topics. The topic is an element to determine customer's behavior and customers' activities are generated according to the topic. In a generative model, customer's behavior is generated with two-step probabilistic process; in the first step a topic is selected according to a topic probability distribution representing topic selection tendency. In the next step user's activity is determined according to activity probability distribution linked to the selected topic in the first step \cite{uetsuji2015}.  




There are some challenges for text recommender system to address, like short term interests vs long term interests users interests, common vs rare interests, content diversity, data sparsity, exploration vs exploitation, and time decay of the interest graph (?)



For news recommendation in digital journals, for example, a majority of users (readers) are anonymous, and frequently news are volatile, they have an extremely short duration while other items arise \cite{diez2016}. Additionally, users' preference for particular articles depends not only on the topic and on propositional content, but also on users' current context. A user's current context can cover various types of information like the user's current location, access time, social environment, and external events (News Rec Sys - NRS 2013). Context-aware recommender systems have been recently studied in order to profile more essential users' preferences with auxiliary context features \cite{kitazawa2016}.



\cite{kumar2017} present a hybrid deep neural model, where a non-linear mapping of users and item features are learnt first. For learning a non-linear mapping for the users, they use an attention-based recurrent layer in combination with fully connected layers. For learning the mappings for the items, they use only fully connected layers. A ranking based objective function is used to learn the parameters of the network. And textual content of the news articles are also used as features for our model. The authors highlight the effectiveness of the model to handle the user cold-start and item cold-start problems.


Current recommendation approaches can be broadly categorized based on their prediction task into missing link prediction methods (what should the user see that he/she has not seen yet?) and next item prediction methods (what are the most likely continuations of the user activity?) \cite{smirnova2017contextual}. 










%Offline evaluation, while useful for comparing recommender performance and gaining understanding into how various algorithms behave, is limited in a variety of ways [88, 89, 98]. It is limited to operating on data regarding past behavior, measuring only the ability to recommend items the user found somehow. Further, there is a selection bias in historical rating data, as users are more likely to consume and therefore be able to rate items they perceive to be good. Time-based methods compensate for this somewhat, but offline evaluations are incapable of measuring the recommender?s ability to recommend good items that the user did not eventually find somehow. They also cannot measure how users respond to recommendations or how recommendations impact business concerns \cite{Ekstrand2011}. 
%
%Recommendation algorithms with similar numeric performance have been known to return observably different results [97, 146], and a decrease in error may or may not make the system better at meeting the user?s needs. The only way to accurately assess these factors is to do an online evaluation ? to try a system with real users \cite{Ekstrand2011}.
%
%Since recommendation is usually a means to some other goal (user satisfaction, increased sales), testing ultimately needs to take this into account and measure the intended effect. However, it can be costly to try algorithms on real sets of users and measure the effects \cite{Shani2010}. 
%
%Online evaluations come in a variety of forms. Field trials ? where a recommender is deployed in a live system and the users? subsequent interactions with the system are recorded ? enable the designer to see how users interact with the recommender and change their behavior in ?real? environments \cite{Ekstrand2011}. 
%
%Since many recommenders are provided in web-based contexts, page views, interface clicks, rating behavior, and purchase behavior can be measured and used to assess the impact of the recommender. Field trials, frequently in the form of A/B tests, are commonly used in commercial recommender deployments where sites have already established user bases and can test a new algorithm or other site change on a small subset of their users [76, 77]. Amazon and Google are well-known for using A/B testing in refining and evaluating their services. Field trials can also be used to measure other aspects of system performance such as recommender accuracy in response to a change in the system [117] \cite{Ekstrand2011}. 
%
%When combined with user surveys, they can be used to assess user satisfaction and other subjective qualities. Recommender effectiveness with respect to business concerns can also be measured in field trials using a variety of measurements used to evaluate marketing campaigns [31] \cite{Ekstrand2011}.
%
%Virtual lab studies are another common method for evaluating recommender systems. They can be used without access to a live user base, and are therefore useful for testing new ideas for which no deployed application exists or is available. They generally have a small number of users who are invited to participate, and can take the form of inter- action with a full application [19] or a survey structured around the recommender [29, 39, 118, 146]. 
%
%Many uses of online evaluation, such as measuring accepted recommendations, page views, conversions, or sales lift, are well-understood. Well-constructed surveys can help get at many other aspects of recommender quality and utility \cite{Ekstrand2011}. 
%
%Determining ways to measure more subtle aspects of recommender quality and user satisfaction is the subject of ongoing research. Shani and Gunawardana \cite{Shani2010} describe many aspects of online and offline evaluations, and more work is needed to come up with good ways to assess recommender's ability to meet user's needs. User Information Needs discusses in more detail what some of these needs are and surveys research on addressing them \cite{Ekstrand2011}.





\subsection{Architectures of Deep Learning}

Depending on how the architectures are intended for use, deep learning can be categorized into Generative or Discriminative deep architectures.

Generative deep architectures models the high-order correlation properties of the observed data for pattern analysis or synthesis purposes, and also characterizes the joint statistical distributions of the observed data and their associated classes. In the latter case, the use of Bayes rule can turn this type of architecture into a discriminative one \cite{bengio2009} \cite{heigold2011} \cite{lecun2007} \cite{zheng2016} \cite{deng2014book} \cite{betru2017}. 

Discriminative deep architectures are intended to directly provide discrimination power for pattern classification, often by characterizing the posterior distributions of classes conditioned on the visible data \cite{bengio2009} \cite{heigold2011} \cite{lecun2007} \cite{zheng2016} \cite{deng2014book} \cite{betru2017}.

In Hybrid deep architectures, the goal is discrimination, but assisted (often in a significant way) with the outcomes of generative architectures via better optimization or/and regularization. On the other hand, discriminative criteria might be used to learn the parameters in any of the deep generative models \cite{bengio2009} \cite{heigold2011} \cite{lecun2007} \cite{zheng2016} \cite{deng2014book} \cite{betru2017}.

